Examining transitional galaxies to understand the role of clusters and their dynamical status in galaxy quenching

In this work, we consider four different galaxy populations and two distinct global environments in the local Universe (z $\leq 0.11$) to investigate the evolution of transitional galaxies (such as star-forming spheroids and passive discs) across different environments. Our sample is composed of 3,899 galaxies within the R$_{200}$ radius of 231 clusters and 11,460 field galaxies. We also investigate the impact of the cluster's dynamic state, as well as the galaxy's location in the projected phase space diagram (PPS). We found that although the cluster environment as a whole influences galaxy evolution, the cluster dynamical state does not. Furthermore, star-forming galaxies represent recent cluster arrivals in comparison to passive galaxies (especially in the case of early-types). Among the ETGs, we find that the D$_n(4000)$ and H$_\delta$ parameters indicate a smooth transition between the subpopulations. In particular, for the SF-ETGs, we detect a significant difference between field and cluster galaxies, as a function of stellar mass, for objects with Log $M_*$/M$_{\odot} > 10.5$. Analyzing the color gradient, the results point toward a picture where field galaxies are more likely to follow the monolithic scenario, while the cluster galaxies the hierarchical scenario. In particular, if we split the ETGs into lenticulars and ellipticals, we find that the steeper color gradients are more common for the lenticulars. Finally, our results indicate the need for galaxy pre-processing in smaller groups, before entering clusters.

==> biblio.tex <==
%% The BibTeX bibliography file was created manually by Laurie Riguccini

%% Created by Laurie Riguccini on June 13th 2017 


%% Saved with string encoding Unicode (UTF-8) 

% Introdução
@ARTICLE{strateva+01,
       author = {{Strateva}, Iskra and {Ivezi{\'c}}, {\v{Z}}eljko and {Knapp}, Gillian R. and {Narayanan}, Vijay K. and {Strauss}, Michael A. and {Gunn}, James E. and {Lupton}, Robert H. and {Schlegel}, David and {Bahcall}, Neta A. and {Brinkmann}, Jon and {Brunner}, Robert J. and {Budav{\'a}ri}, Tam{\'a}s and {Csabai}, Istv{\'a}n and {Castander}, Francisco Javier and {Doi}, Mamoru and {Fukugita}, Masataka and {Gy{\H{o}}ry}, Zsuzsanna and {Hamabe}, Masaru and {Hennessy}, Greg and {Ichikawa}, Takashi and {Kunszt}, Peter Z. and {Lamb}, Don Q. and {McKay}, Timothy A. and {Okamura}, Sadanori and {Racusin}, Judith and {Sekiguchi}, Maki and {Schneider}, Donald P. and {Shimasaku}, Kazuhiro and {York}, Donald},
        title = "{Color Separation of Galaxy Types in the Sloan Digital Sky Survey Imaging Data}",
      journal = {\aj},
     keywords = {Galaxies: Fundamental Parameters, Astrophysics},
         year = 2001,
        month = oct,
       volume = {122},
       number = {4},
        pages = {1861-1874},
          doi = {10.1086/323301},
archivePrefix = {arXiv},
       eprint = {astro-ph/0107201},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001AJ....122.1861S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{baldry+04,
       author = {{Baldry}, Ivan K. and {Glazebrook}, Karl and {Brinkmann}, Jon and {Ivezi{\'c}}, {\v{Z}}eljko and {Lupton}, Robert H. and {Nichol}, Robert C. and {Szalay}, Alexander S.},
        title = "{Quantifying the Bimodal Color-Magnitude Distribution of Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Luminosity Function, Mass Function, Galaxies: Photometry, Astrophysics},
         year = 2004,
        month = jan,
       volume = {600},
       number = {2},
        pages = {681-694},
          doi = {10.1086/380092},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309710},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...600..681B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baldry+06,
       author = {{Baldry}, I.~K. and {Balogh}, M.~L. and {Bower}, R.~G. and {Glazebrook}, K. and {Nichol}, R.~C. and {Bamford}, S.~P. and {Budavari}, T.},
        title = "{Galaxy bimodality versus stellar mass and environment}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: luminosity function, mass function, Astrophysics},
         year = 2006,
        month = dec,
       volume = {373},
       number = {2},
        pages = {469-483},
          doi = {10.1111/j.1365-2966.2006.11081.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0607648},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.373..469B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balogh+04,
       author = {{Balogh}, Michael L. and {Baldry}, Ivan K. and {Nichol}, Robert and {Miller}, Chris and {Bower}, Richard and {Glazebrook}, Karl},
        title = "{The Bimodal Galaxy Color Distribution: Dependence on Luminosity and Environment}",
      journal = {\apjl},
     keywords = {Galaxies: Clusters: General, Galaxies: Evolution, Astrophysics},
         year = 2004,
        month = nov,
       volume = {615},
       number = {2},
        pages = {L101-L104},
          doi = {10.1086/426079},
archivePrefix = {arXiv},
       eprint = {astro-ph/0406266},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...615L.101B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dressler1980,
       author = {{Dressler}, A.},
        title = "{Galaxy morphology in rich clusters: implications for the formation and evolution of galaxies.}",
      journal = {\apj},
     keywords = {Elliptical Galaxies, Galactic Clusters, Galactic Evolution, Galactic Structure, Spiral Galaxies, Astronomical Maps, Density Distribution, Interstellar Gas, Telescopes, Universe, X Ray Astronomy, Astrophysics},
         year = 1980,
        month = mar,
       volume = {236},
        pages = {351-365},
          doi = {10.1086/157753},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980ApJ...236..351D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{butcher&oemler84,
       author = {{Butcher}, H. and {Oemler}, A., Jr.},
        title = "{The evolution of galaxies in clusters. V. A study of populations since Z 0.5.}",
      journal = {\apj},
     keywords = {Astronomical Photometry, Cosmology, Galactic Clusters, Galactic Evolution, Red Shift, Colorimetry, Spiral Galaxies, Virgo Galactic Cluster, Astrophysics},
         year = 1984,
        month = oct,
       volume = {285},
        pages = {426-438},
          doi = {10.1086/162519},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984ApJ...285..426B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wolf+09,
       author = {{Wolf}, Christian and {Arag{\'o}n-Salamanca}, Alfonso and {Balogh}, Michael and {Barden}, Marco and {Bell}, Eric F. and {Gray}, Meghan E. and {Peng}, Chien Y. and {Bacon}, David and {Barazza}, Fabio D. and {B{\"o}hm}, Asmus and {Caldwell}, John A.~R. and {Gallazzi}, Anna and {H{\"a}u{\ss}ler}, Boris and {Heymans}, Catherine and {Jahnke}, Knud and {Jogee}, Shardha and {van Kampen}, Eelco and {Lane}, Kyle and {McIntosh}, Daniel H. and {Meisenheimer}, Klaus and {Papovich}, Casey and {S{\'a}nchez}, Sebastian F. and {Taylor}, Andy and {Wisotzki}, Lutz and {Zheng}, Xianzhong},
        title = "{The STAGES view of red spirals and dusty red galaxies: mass-dependent quenching of star formation in cluster infall}",
      journal = {\mnras},
     keywords = {surveys, stars: formation, galaxies: clusters: general, galaxies: evolution, galaxies: spiral, infrared: galaxies, Astrophysics},
         year = 2009,
        month = mar,
       volume = {393},
       number = {4},
        pages = {1302-1323},
          doi = {10.1111/j.1365-2966.2008.14204.x},
archivePrefix = {arXiv},
       eprint = {0811.3873},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.393.1302W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{crossett+14,
       author = {{Crossett}, Jacob P. and {Pimbblet}, Kevin A. and {Stott}, John P. and {Jones}, D. Heath},
        title = "{Environments and morphologies of red sequence galaxies with residual star formation in massive clusters}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: stellar content, ultraviolet: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = jan,
       volume = {437},
       number = {3},
        pages = {2521-2530},
          doi = {10.1093/mnras/stt2065},
archivePrefix = {arXiv},
       eprint = {1310.7602},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.437.2521C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cortese12,
       author = {{Cortese}, L.},
        title = "{Are passive red spirals truly passive?. The current star formation activity of optically red disc galaxies}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: photometry, galaxies: star formation, ultraviolet: galaxies, infrared: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = jul,
       volume = {543},
          eid = {A132},
        pages = {A132},
          doi = {10.1051/0004-6361/201219443},
archivePrefix = {arXiv},
       eprint = {1205.6819},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...543A.132C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{masters+10,
       author = {{Masters}, Karen L. and {Mosleh}, Moein and {Romer}, A. Kathy and {Nichol}, Robert C. and {Bamford}, Steven P. and {Schawinski}, Kevin and {Lintott}, Chris J. and {Andreescu}, Dan and {Campbell}, Heather C. and {Crowcroft}, Ben and {Doyle}, Isabelle and {Edmondson}, Edward M. and {Murray}, Phil and {Raddick}, M. Jordan and {Slosar}, An{\v{z}}e and {Szalay}, Alexander S. and {Vandenberg}, Jan},
        title = "{Galaxy Zoo: passive red spirals}",
      journal = {\mnras},
     keywords = {surveys, galaxies: active, galaxies: evolution, galaxies: photometry, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = jun,
       volume = {405},
       number = {2},
        pages = {783-799},
          doi = {10.1111/j.1365-2966.2010.16503.x},
archivePrefix = {arXiv},
       eprint = {0910.4113},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.405..783M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lopes+16,
       author = {{Lopes}, P.~A.~A. and {Rembold}, S.~B. and {Ribeiro}, A.~L.~B. and {Nascimento}, R.~S. and {Vajgel}, B.},
        title = "{NoSOCS in SDSS - V. Red disc and blue bulge galaxies across different environments}",
      journal = {\mnras},
     keywords = {surveys, galaxies: clusters: general, galaxies: evolution, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = sep,
       volume = {461},
       number = {3},
        pages = {2559-2579},
          doi = {10.1093/mnras/stw1497},
archivePrefix = {arXiv},
       eprint = {1606.06280},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.461.2559L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martin+07,
       author = {{Martin}, D. Christopher and {Wyder}, Ted K. and {Schiminovich}, David and {Barlow}, Tom A. and {Forster}, Karl and {Friedman}, Peter G. and {Morrissey}, Patrick and {Neff}, Susan G. and {Seibert}, Mark and {Small}, Todd and {Welsh}, Barry Y. and {Bianchi}, Luciana and {Donas}, Jos{\'e} and {Heckman}, Timothy M. and {Lee}, Young-Wook and {Madore}, Barry F. and {Milliard}, Bruno and {Rich}, R. Michael and {Szalay}, Alex S. and {Yi}, Sukyoung K.},
        title = "{The UV-Optical Galaxy Color-Magnitude Diagram. III. Constraints on Evolution from the Blue to the Red Sequence}",
      journal = {\apjs},
     keywords = {Galaxies: Evolution, Ultraviolet: Galaxies, Astrophysics},
         year = 2007,
        month = dec,
       volume = {173},
       number = {2},
        pages = {342-356},
          doi = {10.1086/516639},
archivePrefix = {arXiv},
       eprint = {astro-ph/0703281},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJS..173..342M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{salim+09,
       author = {{Salim}, Samir and {Dickinson}, Mark and {Michael Rich}, R. and {Charlot}, St{\'e}phane and {Lee}, Janice C. and {Schiminovich}, David and {P{\'e}rez-Gonz{\'a}lez}, Pablo G. and {Ashby}, Matthew L.~N. and {Papovich}, Casey and {Faber}, S.~M. and {Ivison}, Rob J. and {Frayer}, David T. and {Walton}, Josiah M. and {Weiner}, Benjamin J. and {Chary}, Ranga-Ram and {Bundy}, Kevin and {Noeske}, Kai and {Koekemoer}, Anton M.},
        title = "{Mid-IR Luminosities and UV/Optical Star Formation Rates at z < 1.4}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: evolution, galaxies: fundamental parameters, infrared: galaxies, surveys, ultraviolet: galaxies, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2009,
        month = jul,
       volume = {700},
       number = {1},
        pages = {161-182},
          doi = {10.1088/0004-637X/700/1/161},
archivePrefix = {arXiv},
       eprint = {0905.0162},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...700..161S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mendez+11,
       author = {{Mendez}, Alexander J. and {Coil}, Alison L. and {Lotz}, Jennifer and {Salim}, Samir and {Moustakas}, John and {Simard}, Luc},
        title = "{AEGIS: The Morphologies of Green Galaxies at 0.4 < z < 1.2}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: statistics, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = aug,
       volume = {736},
       number = {2},
          eid = {110},
        pages = {110},
          doi = {10.1088/0004-637X/736/2/110},
archivePrefix = {arXiv},
       eprint = {1101.3353},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...736..110M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schawinski+14,
       author = {{Schawinski}, Kevin and {Urry}, C. Megan and {Simmons}, Brooke D. and {Fortson}, Lucy and {Kaviraj}, Sugata and {Keel}, William C. and {Lintott}, Chris J. and {Masters}, Karen L. and {Nichol}, Robert C. and {Sarzi}, Marc and {Skibba}, Ramin and {Treister}, Ezequiel and {Willett}, Kyle W. and {Wong}, O. Ivy and {Yi}, Sukyoung K.},
        title = "{The green valley is a red herring: Galaxy Zoo reveals two evolutionary pathways towards quenching of star formation in early- and late-type galaxies}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: spiral, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = may,
       volume = {440},
       number = {1},
        pages = {889-907},
          doi = {10.1093/mnras/stu327},
archivePrefix = {arXiv},
       eprint = {1402.4814},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.440..889S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gunn&gott-72,
       author = {{Gunn}, James E. and {Gott}, J. Richard, III},
        title = "{On the Infall of Matter Into Clusters of Galaxies and Some Effects on Their Evolution}",
      journal = {\apj},
         year = 1972,
        month = aug,
       volume = {176},
        pages = {1},
          doi = {10.1086/151605},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...176....1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{larson+80,
       author = {{Larson}, R.~B. and {Tinsley}, B.~M. and {Caldwell}, C.~N.},
        title = "{The evolution of disk galaxies and the origin of S0 galaxies}",
      journal = {\apj},
     keywords = {Disk Galaxies, Galactic Evolution, Spiral Galaxies, Digital Simulation, Galactic Structure, Gas Evolution, Stellar Evolution, Stellar Magnitude, Astrophysics},
         year = 1980,
        month = may,
       volume = {237},
        pages = {692-707},
          doi = {10.1086/157917},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980ApJ...237..692L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{toomre&toomre-72,
       author = {{Toomre}, Alar and {Toomre}, Juri},
        title = "{Galactic Bridges and Tails}",
      journal = {\apj},
         year = 1972,
        month = dec,
       volume = {178},
        pages = {623-666},
          doi = {10.1086/151823},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972ApJ...178..623T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moore+96,
       author = {{Moore}, Ben and {Katz}, Neal and {Lake}, George and {Dressler}, Alan and {Oemler}, Augustus},
        title = "{Galaxy harassment and the evolution of clusters of galaxies}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 1996,
        month = feb,
       volume = {379},
       number = {6566},
        pages = {613-616},
          doi = {10.1038/379613a0},
archivePrefix = {arXiv},
       eprint = {astro-ph/9510034},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996Natur.379..613M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moore+98,
       author = {{Moore}, Ben and {Lake}, George and {Katz}, Neal},
        title = "{Morphological Transformation from Galaxy Harassment}",
      journal = {\apj},
     keywords = {GALAXIES: EVOLUTION, GALAXIES: INTERACTIONS, GALAXIES: STARBURST, GALAXIES: STRUCTURE, METHODS: NUMERICAL, Galaxies: Evolution, Galaxies: Interactions, Galaxies: Starburst, Galaxies: Structure, Methods: Numerical, Astrophysics},
         year = 1998,
        month = mar,
       volume = {495},
       number = {1},
        pages = {139-151},
          doi = {10.1086/305264},
archivePrefix = {arXiv},
       eprint = {astro-ph/9701211},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...495..139M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{byrd&valtonen-01,
       author = {{Byrd}, Gene and {Valtonen}, Mauri},
        title = "{Tides and Markarian Activity in Karachentsev Disk Galaxy Pairs}",
      journal = {\aj},
     keywords = {Galaxies: Binary, Galaxies: Interactions, Galaxies: Seyfert, Galaxies: Spiral, Galaxies: Statistics},
         year = 2001,
        month = jun,
       volume = {121},
       number = {6},
        pages = {2943-2949},
          doi = {10.1086/321089},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001AJ....121.2943B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lokas+16,
       author = {{{\L}okas}, Ewa L. and {Ebrov{\'a}}, Ivana and {del Pino}, Andr{\'e}s and {Sybilska}, Agnieszka and {Athanassoula}, E. and {Semczuk}, Marcin and {Gajda}, Grzegorz and {Fouquet}, Sylvain},
        title = "{Tidally Induced Bars of Galaxies in Clusters}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: fundamental parameters, galaxies: interactions, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = aug,
       volume = {826},
       number = {2},
          eid = {227},
        pages = {227},
          doi = {10.3847/0004-637X/826/2/227},
archivePrefix = {arXiv},
       eprint = {1601.07433},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826..227L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ponman+99,
       author = {{Ponman}, Trevor J. and {Cannon}, Damian B. and {Navarro}, Julio F.},
        title = "{The thermal imprint of galaxy formation on X-ray clusters}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 1999,
        month = jan,
       volume = {397},
       number = {6715},
        pages = {135-137},
          doi = {10.1038/16410},
archivePrefix = {arXiv},
       eprint = {astro-ph/9810359},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999Natur.397..135P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{larson74,
       author = {{Larson}, Richard B.},
        title = "{Effects of supernovae on the early evolution of galaxies}",
      journal = {\mnras},
         year = 1974,
        month = nov,
       volume = {169},
        pages = {229-246},
          doi = {10.1093/mnras/169.2.229},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974MNRAS.169..229L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vecchia+08,
       author = {{Dalla Vecchia}, Claudio and {Schaye}, Joop},
        title = "{Simulating galactic outflows with kinetic supernova feedback}",
      journal = {\mnras},
     keywords = {methods: numerical, ISM: bubbles, ISM: jets and outflows, galaxies: evolution, galaxies: formation, galaxies: ISM, Astrophysics},
         year = 2008,
        month = jul,
       volume = {387},
       number = {4},
        pages = {1431-1444},
          doi = {10.1111/j.1365-2966.2008.13322.x},
archivePrefix = {arXiv},
       eprint = {0801.2770},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.387.1431D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{coton+06,
       author = {{Croton}, Darren J. and {Springel}, Volker and {White}, Simon D.~M. and {De Lucia}, G. and {Frenk}, C.~S. and {Gao}, L. and {Jenkins}, A. and {Kauffmann}, G. and {Navarro}, J.~F. and {Yoshida}, N.},
        title = "{The many lives of active galactic nuclei: cooling flows, black holes and the luminosities and colours of galaxies}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, cooling flows, galaxies: evolution, galaxies: formation, cosmology: theory, Astrophysics},
         year = 2006,
        month = jan,
       volume = {365},
       number = {1},
        pages = {11-28},
          doi = {10.1111/j.1365-2966.2005.09675.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508046},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.365...11C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fabian+12,
       author = {{Fabian}, A.~C.},
        title = "{Observational Evidence of Active Galactic Nuclei Feedback}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = sep,
       volume = {50},
        pages = {455-489},
          doi = {10.1146/annurev-astro-081811-125521},
archivePrefix = {arXiv},
       eprint = {1204.4114},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ARA&A..50..455F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{peng10,
       author = {{Peng}, Ying-jie and {Lilly}, Simon J. and {Kova{\v{c}}}, Katarina and {Bolzonella}, Micol and {Pozzetti}, Lucia and {Renzini}, Alvio and {Zamorani}, Gianni and {Ilbert}, Olivier and {Knobel}, Christian and {Iovino}, Angela and {Maier}, Christian and {Cucciati}, Olga and {Tasca}, Lidia and {Carollo}, C. Marcella and {Silverman}, John and {Kampczyk}, Pawel and {de Ravel}, Loic and {Sanders}, David and {Scoville}, Nicholas and {Contini}, Thierry and {Mainieri}, Vincenzo and {Scodeggio}, Marco and {Kneib}, Jean-Paul and {Le F{\`e}vre}, Olivier and {Bardelli}, Sandro and {Bongiorno}, Angela and {Caputi}, Karina and {Coppa}, Graziano and {de la Torre}, Sylvain and {Franzetti}, Paolo and {Garilli}, Bianca and {Lamareille}, Fabrice and {Le Borgne}, Jean-Francois and {Le Brun}, Vincent and {Mignoli}, Marco and {Perez Montero}, Enrique and {Pello}, Roser and {Ricciardelli}, Elena and {Tanaka}, Masayuki and {Tresse}, Laurence and {Vergani}, Daniela and {Welikala}, Niraj and {Zucca}, Elena and {Oesch}, Pascal and {Abbas}, Ummi and {Barnes}, Luke and {Bordoloi}, Rongmon and {Bottini}, Dario and {Cappi}, Alberto and {Cassata}, Paolo and {Cimatti}, Andrea and {Fumana}, Marco and {Hasinger}, Gunther and {Koekemoer}, Anton and {Leauthaud}, Alexei and {Maccagni}, Dario and {Marinoni}, Christian and {McCracken}, Henry and {Memeo}, Pierdomenico and {Meneux}, Baptiste and {Nair}, Preethi and {Porciani}, Cristiano and {Presotto}, Valentina and {Scaramella}, Roberto},
        title = "{Mass and Environment as Drivers of Galaxy Evolution in SDSS and zCOSMOS and the Origin of the Schechter Function}",
      journal = {\apj},
     keywords = {cosmology: observations, galaxies: active, galaxies: distances and redshifts, galaxies: evolution, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2010,
        month = sep,
       volume = {721},
       number = {1},
        pages = {193-221},
          doi = {10.1088/0004-637X/721/1/193},
archivePrefix = {arXiv},
       eprint = {1003.4747},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...721..193P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jaffe+15,
       author = {{Jaff{\'e}}, Yara L. and {Smith}, Rory and {Candlish}, Graeme N. and {Poggianti}, Bianca M. and {Sheen}, Yun-Kyeong and {Verheijen}, Marc A.~W.},
        title = "{BUDHIES II: a phase-space view of H I gas stripping and star formation quenching in cluster galaxies}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: clusters: invidivual: Abell 963, galaxies: clusters: intracluster medium, galaxies: evolution, galaxies: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = apr,
       volume = {448},
       number = {2},
        pages = {1715-1728},
          doi = {10.1093/mnras/stv100},
archivePrefix = {arXiv},
       eprint = {1501.03819},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.448.1715J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
%-------------------------------------------------------------------
% Data
%-------------------------------------------------------------------
@ARTICLE{Lopes+04,
       author = {{Lopes}, P.~A.~A. and {de Carvalho}, R.~R. and {Gal}, R.~R. and {Djorgovski}, S.~G. and {Odewahn}, S.~C. and {Mahabal}, A.~A. and {Brunner}, R.~J.},
        title = "{The Northern Sky Optical Cluster Survey. IV. An Intermediate-Redshift Galaxy Cluster Catalog and the Comparison of Two Detection Algorithms}",
      journal = {\aj},
     keywords = {Galaxies: Clusters: General, Methods: Numerical, Surveys},
         year = 2004,
        month = sep,
       volume = {128},
       number = {3},
        pages = {1017-1045},
          doi = {10.1086/423038},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004AJ....128.1017L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lop09a,
       author = {{Lopes}, P.~A.~A. and {de Carvalho}, R.~R. and {Kohl-Moreira}, J.~L. and {Jones}, C.},
        title = "{NoSOCS in SDSS - I. Sample definition and comparison of mass estimates}",
      journal = {\mnras},
     keywords = {surveys, galaxies: clusters: general, galaxies: kinematics and dynamics, Astrophysics},
         year = 2009,
        month = jan,
       volume = {392},
       number = {1},
        pages = {135-152},
          doi = {10.1111/j.1365-2966.2008.13962.x},
archivePrefix = {arXiv},
       eprint = {0809.2595},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.392..135L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lop09b,
   author = {{Lopes}, P.~A.~A. and {de Carvalho}, R.~R. and {Kohl-Moreira}, J.~L. and 
	{Jones}, C.},
    title = "{NoSOCS in SDSS - II. Mass calibration of low redshift galaxy clusters with optical and X-ray properties}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0907.3753},
 primaryClass = "astro-ph.CO",
 keywords = {surveys , galaxies: clusters: general , galaxies: kinematics and dynamics},
     year = 2009,
    month = nov,
   volume = 399,
    pages = {2201-2220},
      doi = {10.1111/j.1365-2966.2009.15425.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399.2201L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spiders,
       author = {{Dwelly}, T. and {Salvato}, M. and {Merloni}, A. and {Brusa}, M. and {Buchner}, J. and {Anderson}, S.~F. and {Boller}, Th. and {Brandt}, W.~N. and {Budav{\'a}ri}, T. and {Clerc}, N. and {Coffey}, D. and {Del Moro}, A. and {Georgakakis}, A. and {Green}, P.~J. and {Jin}, C. and {Menzel}, M. -L. and {Myers}, A.~D. and {Nandra}, K. and {Nichol}, R.~C. and {Ridl}, J. and {Schwope}, A.~D. and {Simm}, T.},
        title = "{SPIDERS: selection of spectroscopic targets using AGN candidates detected in all-sky X-ray surveys}",
      journal = {\mnras},
     keywords = {surveys, galaxies: active, quasars: general, galaxies: Seyfert, cosmology: observations, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jul,
       volume = {469},
       number = {1},
        pages = {1065-1095},
          doi = {10.1093/mnras/stx864},
archivePrefix = {arXiv},
       eprint = {1704.01796},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.469.1065D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andrade-Santos+17,
       author = {{Andrade-Santos}, Felipe and {Jones}, Christine and {Forman}, William R. and {Lovisari}, Lorenzo and {Vikhlinin}, Alexey and {van Weeren}, Reinout J. and {Murray}, Stephen S. and {Arnaud}, Monique and {Pratt}, Gabriel W. and {D{\'e}mocl{\`e}s}, Jessica and {Kraft}, Ralph and {Mazzotta}, Pasquale and {B{\"o}hringer}, Hans and {Chon}, Gayoung and {Giacintucci}, Simona and {Clarke}, Tracy E. and {Borgani}, Stefano and {David}, Larry and {Douspis}, Marian and {Pointecouteau}, Etienne and {Dahle}, H{\r{a}}kon and {Brown}, Shea and {Aghanim}, Nabila and {Rasia}, Elena},
        title = "{The Fraction of Cool-core Clusters in X-Ray versus SZ Samples Using Chandra Observations}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, large-structure of universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = jul,
       volume = {843},
       number = {1},
          eid = {76},
        pages = {76},
          doi = {10.3847/1538-4357/aa7461},
archivePrefix = {arXiv},
       eprint = {1703.08690},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843...76A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fadda+96,
       author = {{Fadda}, D. and {Girardi}, M. and {Giuricin}, G. and {Mardirossian}, F. and {Mezzetti}, M.},
        title = "{The Observational Distribution of Internal Velocity Dispersions in Nearby Galaxy Clusters}",
      journal = {\apj},
     keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: DISTANCES AND REDSHIFTS, GALAXIES: KINEMATICS AND DYNAMICS, Astrophysics},
         year = 1996,
        month = dec,
       volume = {473},
        pages = {670},
          doi = {10.1086/178180},
archivePrefix = {arXiv},
       eprint = {astro-ph/9606098},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...473..670F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%paulo+14
@ARTICLE{Lopes+14,
       author = {{Lopes}, P.~A.~A. and {Ribeiro}, A.~L.~B. and {Rembold}, S.~B.},
        title = "{NoSOCS in SDSS - IV. The role of environment beyond the extent of galaxy clusters}",
      journal = {\mnras},
     keywords = {surveys, galaxies: evolution, galaxies: clusters: environment, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2014,
        month = jan,
       volume = {437},
       number = {3},
        pages = {2430-2447},
          doi = {10.1093/mnras/stt2064},
archivePrefix = {arXiv},
       eprint = {1310.6309},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.437.2430L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{trussler+20,
       author = {{Trussler}, James and {Maiolino}, Roberto and {Maraston}, Claudia and {Peng}, Yingjie and {Thomas}, Daniel and {Goddard}, Daniel and {Lian}, Jianhui},
        title = "{Both starvation and outflows drive galaxy quenching}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = feb,
       volume = {491},
       number = {4},
        pages = {5406-5434},
          doi = {10.1093/mnras/stz3286},
archivePrefix = {arXiv},
       eprint = {1811.09283},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.5406T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%paulo+18
@ARTICLE{Lopes+18,
       author = {{Lopes}, Paulo A.~A. and {Trevisan}, M. and {Lagan{\'a}}, T.~F. and {Durret}, F. and {Ribeiro}, A.~L.~B. and {Rembold}, S.~B.},
        title = "{Optical substructure and BCG offsets of Sunyaev-Zel'dovich and X-ray-selected galaxy clusters}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: clusters: intracluster medium, X-rays: galaxies: clusters, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = aug,
       volume = {478},
       number = {4},
        pages = {5473-5490},
          doi = {10.1093/mnras/sty1374},
archivePrefix = {arXiv},
       eprint = {1805.09631},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.478.5473L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brinchmann+04,
       author = {{Brinchmann}, J. and {Charlot}, S. and {White}, S.~D.~M. and {Tremonti}, C. and {Kauffmann}, G. and {Heckman}, T. and {Brinkmann}, J.},
        title = "{The physical properties of star-forming galaxies in the low-redshift Universe}",
      journal = {\mnras},
     keywords = {surveys, galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: general, Astrophysics},
         year = 2004,
        month = jul,
       volume = {351},
       number = {4},
        pages = {1151-1179},
          doi = {10.1111/j.1365-2966.2004.07881.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0311060},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.351.1151B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kau03a,
       author = {{Kauffmann}, Guinevere and {Heckman}, Timothy M. and {White}, Simon D.~M. and {Charlot}, St{\'e}phane and {Tremonti}, Christy and {Brinchmann}, Jarle and {Bruzual}, Gustavo and {Peng}, Eric W. and {Seibert}, Mark and {Bernardi}, Mariangela and {Blanton}, Michael and {Brinkmann}, Jon and {Castander}, Francisco and {Cs{\'a}bai}, Istvan and {Fukugita}, Masataka and {Ivezic}, Zeljko and {Munn}, Jeffrey A. and {Nichol}, Robert C. and {Padmanabhan}, Nikhil and {Thakar}, Aniruddha R. and {Weinberg}, David H. and {York}, Donald},
        title = "{Stellar masses and star formation histories for {}10$^{5}$ galaxies from the Sloan Digital Sky Survey}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = may,
       volume = {341},
       number = {1},
        pages = {33-53},
          doi = {10.1046/j.1365-8711.2003.06291.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0204055},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.341...33K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremonti+04,
       author = {{Tremonti}, Christy A. and {Heckman}, Timothy M. and {Kauffmann}, Guinevere and {Brinchmann}, Jarle and {Charlot}, St{\'e}phane and {White}, Simon D.~M. and {Seibert}, Mark and {Peng}, Eric W. and {Schlegel}, David J. and {Uomoto}, Alan and {Fukugita}, Masataka and {Brinkmann}, Jon},
        title = "{The Origin of the Mass-Metallicity Relation: Insights from 53,000 Star-forming Galaxies in the Sloan Digital Sky Survey}",
      journal = {\apj},
     keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Statistics, Astrophysics},
         year = 2004,
        month = oct,
       volume = {613},
       number = {2},
        pages = {898-913},
          doi = {10.1086/423264},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405537},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...613..898T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dominguez-Sanchez+18,
       author = {{Dom{\'\i}nguez S{\'a}nchez}, H. and {Huertas-Company}, M. and {Bernardi}, M. and {Tuccillo}, D. and {Fischer}, J.~L.},
        title = "{Improving galaxy morphologies for SDSS with Deep Learning}",
      journal = {\mnras},
     keywords = {methods: observational, catalogues, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = feb,
       volume = {476},
       number = {3},
        pages = {3661-3676},
          doi = {10.1093/mnras/sty338},
archivePrefix = {arXiv},
       eprint = {1711.05744},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476.3661D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Huertas-Company+11,
       author = {{Huertas-Company}, M. and {Aguerri}, J.~A.~L. and {Bernardi}, M. and {Mei}, S. and {S{\'a}nchez Almeida}, J.},
        title = "{Revisiting the Hubble sequence in the SDSS DR7 spectroscopic sample: a publicly available Bayesian automated classification}",
      journal = {\aap},
     keywords = {catalogs, astronomical databases: miscellaneous, Galaxy: fundamental parameters, galaxies: evolution, Galaxy: formation, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jan,
       volume = {525},
          eid = {A157},
        pages = {A157},
          doi = {10.1051/0004-6361/201015735},
archivePrefix = {arXiv},
       eprint = {1010.3018},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...525A.157H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gal09,
       author = {{Gal}, R.~R. and {Lopes}, P.~A.~A. and {de Carvalho}, R.~R. and {Kohl-Moreira}, J.~L. and {Capelato}, H.~V. and {Djorgovski}, S.~G.},
        title = "{The Northern Sky Optical Cluster Survey. III. A Cluster Catalog Covering PI Steradians}",
      journal = {\aj},
     keywords = {catalogs, galaxies: clusters: general, large-scale structure of universe, surveys, Astrophysics},
         year = 2009,
        month = feb,
       volume = {137},
       number = {2},
        pages = {2981-2999},
          doi = {10.1088/0004-6256/137/2/2981},
archivePrefix = {arXiv},
       eprint = {0812.2962},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009AJ....137.2981G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

% subsection: cluster dynamical state
@ARTICLE{dressler-shctman_88,
       author = {{Dressler}, Alan and {Shectman}, Stephen A.},
        title = "{Evidence for Substructure in Rich Clusters of Galaxies from Radial-Velocity Measurements}",
      journal = {\aj},
     keywords = {Galactic Clusters, Radial Velocity, Statistical Analysis, Velocity Measurement, Cosmology, Histograms, Astrophysics, GALAXIES: CLUSTERING},
         year = 1988,
        month = apr,
       volume = {95},
        pages = {985},
          doi = {10.1086/114694},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988AJ.....95..985D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%-------------------------------------------------------------------
%       CAP 4
%-------------------------------------------------------------------
@ARTICLE{Mahajan+11,
       author = {{Mahajan}, Smriti and {Mamon}, Gary A. and {Raychaudhury}, Somak},
        title = "{The velocity modulation of galaxy properties in and near clusters: quantifying the decrease in star formation in backsplash galaxies}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: starburst, galaxies: star formation, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2011,
        month = oct,
       volume = {416},
       number = {4},
        pages = {2882-2902},
          doi = {10.1111/j.1365-2966.2011.19236.x},
archivePrefix = {arXiv},
       eprint = {1106.3062},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.416.2882M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Oman+13,
       author = {{Oman}, Kyle A. and {Hudson}, Michael J. and {Behroozi}, Peter S.},
        title = "{Disentangling satellite galaxy populations using orbit tracking in simulations}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: haloes, galaxies: kinematics and dynamics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = may,
       volume = {431},
       number = {3},
        pages = {2307-2316},
          doi = {10.1093/mnras/stt328},
archivePrefix = {arXiv},
       eprint = {1301.6757},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.431.2307O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rhee+17,
       author = {{Rhee}, Jinsu and {Smith}, Rory and {Choi}, Hoseung and {Yi}, Sukyoung K. and {Jaff{\'e}}, Yara and {Candlish}, Graeme and {S{\'a}nchez-J{\'a}nssen}, Ruben},
        title = "{Phase-space Analysis in the Group and Cluster Environment: Time Since Infall and Tidal Mass Loss}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: groups: general, galaxies: halos, galaxies: interactions, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jul,
       volume = {843},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.3847/1538-4357/aa6d6c},
archivePrefix = {arXiv},
       eprint = {1704.04243},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843..128R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pasquali+19,
       author = {{Pasquali}, A. and {Smith}, R. and {Gallazzi}, A. and {De Lucia}, G. and {Zibetti}, S. and {Hirschmann}, M. and {Yi}, S.~K.},
        title = "{Physical properties of SDSS satellite galaxies in projected phase space}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: general, galaxies: haloes, galaxies: stellar content, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {484},
       number = {2},
        pages = {1702-1723},
          doi = {10.1093/mnras/sty3530},
archivePrefix = {arXiv},
       eprint = {1901.04238},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.1702P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kaviraj+11,
       author = {{Kaviraj}, Sugata and {Tan}, Kok-Meng and {Ellis}, Richard S. and {Silk}, Joseph},
        title = "{A coincidence of disturbed morphology and blue UV colour: minor-merger-driven star formation in early-type galaxies at z{\ensuremath{\sim}} 0.6}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: interactions, ultraviolet: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = mar,
       volume = {411},
       number = {4},
        pages = {2148-2160},
          doi = {10.1111/j.1365-2966.2010.17754.x},
archivePrefix = {arXiv},
       eprint = {1001.2141},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.411.2148K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{marino+09,
       author = {{Marino}, A. and {Iodice}, E. and {Tantalo}, R. and {Piovan}, L. and {Bettoni}, D. and {Buson}, L.~M. and {Chiosi}, C. and {Galletta}, G. and {Rampazzo}, R. and {Rich}, R.~M.},
        title = "{GALEX UV properties of the polar ring galaxy MCG-05-07-001 and the shell galaxies NGC 1210 and NGC 5329}",
      journal = {\aap},
     keywords = {ultraviolet: galaxies, galaxies: elliptical and lenticular, cD, galaxies: individual: MCG-05-07-001, galaxies: evolution, galaxies: individual: NGC 1210, galaxies: NGC 5329, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = dec,
       volume = {508},
       number = {3},
        pages = {1235-1252},
          doi = {10.1051/0004-6361/200911819},
archivePrefix = {arXiv},
       eprint = {0909.4020},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...508.1235M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kaviraj+09,
       author = {{Kaviraj}, Sugata and {Peirani}, Sebastien and {Khochfar}, Sadegh and {Silk}, Joseph and {Kay}, Scott},
        title = "{The role of minor mergers in the recent star formation history of early-type galaxies}",
      journal = {\mnras},
     keywords = {methods: N-body simulations, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, Astrophysics},
         year = 2009,
        month = apr,
       volume = {394},
       number = {4},
        pages = {1713-1720},
          doi = {10.1111/j.1365-2966.2009.14403.x},
archivePrefix = {arXiv},
       eprint = {0711.1493},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.394.1713K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yi+05,
       author = {{Yi}, S.~K. and {Yoon}, S. -J. and {Kaviraj}, S. and {Deharveng}, J. -M. and {Rich}, R.~M. and {Salim}, S. and {Boselli}, A. and {Lee}, Y. -W. and {Ree}, C.~H. and {Sohn}, Y. -J. and {Rey}, S. -C. and {Lee}, J. -W. and {Rhee}, J. and {Bianchi}, L. and {Byun}, Y. -I. and {Donas}, J. and {Friedman}, P.~G. and {Heckman}, T.~M. and {Jelinsky}, P. and {Madore}, B.~F. and {Malina}, R. and {Martin}, D.~C. and {Milliard}, B. and {Morrissey}, P. and {Neff}, S. and {Schiminovich}, D. and {Siegmund}, O. and {Small}, T. and {Szalay}, A.~S. and {Jee}, M.~J. and {Kim}, S. -W. and {Barlow}, T. and {Forster}, K. and {Welsh}, B. and {Wyder}, T.~K.},
        title = "{Galaxy Evolution Explorer Ultraviolet Color-Magnitude Relations and Evidence of Recent Star Formation in Early-Type Galaxies}",
      journal = {\apjl},
     keywords = {Galaxies: Evolution, Galaxies: Formation, Ultraviolet: Galaxies, Astrophysics},
         year = 2005,
        month = jan,
       volume = {619},
       number = {1},
        pages = {L111-L114},
          doi = {10.1086/422811},
archivePrefix = {arXiv},
       eprint = {astro-ph/0411327},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...619L.111Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jaffe+12,
       author = {{Jaff{\'e}}, Yara L. and {Poggianti}, Bianca M. and {Verheijen}, Marc A.~W. and {Deshev}, Boris Z. and {van Gorkom}, Jacqueline H.},
        title = "{Gas Reservoirs and Star Formation in a Forming Galaxy Cluster at zbsime0.2}",
      journal = {\apjl},
     keywords = {galaxies: clusters: general, galaxies: clusters: individual: Abell 2192, galaxies: evolution, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = sep,
       volume = {756},
       number = {2},
          eid = {L28},
        pages = {L28},
          doi = {10.1088/2041-8205/756/2/L28},
archivePrefix = {arXiv},
       eprint = {1207.2767},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...756L..28J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{haines+15,
       author = {{Haines}, C.~P. and {Pereira}, M.~J. and {Smith}, G.~P. and {Egami}, E. and {Babul}, A. and {Finoguenov}, A. and {Ziparo}, F. and {McGee}, S.~L. and {Rawle}, T.~D. and {Okabe}, N. and {Moran}, S.~M.},
        title = "{LoCuSS: The Slow Quenching of Star Formation in Cluster Galaxies and the Need for Pre-processing}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: clusters: general, galaxies: evolution, galaxies: stellar content, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = jun,
       volume = {806},
       number = {1},
          eid = {101},
        pages = {101},
          doi = {10.1088/0004-637X/806/1/101},
archivePrefix = {arXiv},
       eprint = {1504.05604},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...806..101H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mahajan+13,
       author = {{Mahajan}, S.},
        title = "{Evidence for galaxies being pre-processed before accreted into clusters.}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: evolution, X-rays: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = apr,
       volume = {431},
        pages = {L117-L121},
          doi = {10.1093/mnrasl/slt021},
archivePrefix = {arXiv},
       eprint = {1302.2905},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.431L.117M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kias,
       author = {{Choi}, Yun-Young and {Han}, Du-Hwan and {Kim}, Sungsoo S.},
        title = "{Korea Institute for Advanced Study Value-Added Galaxy Catalog}",
      journal = {Journal of Korean Astronomical Society},
     keywords = {galaxies: fundamental parameters, galaxies: general, galaxies: distances and redshifts, catalogs, surveys},
         year = 2010,
        month = dec,
       volume = {43},
       number = {6},
        pages = {191-200},
          doi = {10.5303/JKAS.2010.43.6.191},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010JKAS...43..191C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tortora+10,
       author = {{Tortora}, C. and {Napolitano}, N.~R. and {Cardone}, V.~F. and {Capaccioli}, M. and {Jetzer}, Ph. and {Molinaro}, R.},
        title = "{Colour and stellar population gradients in galaxies: correlation with mass}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: general, dark matter, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = sep,
       volume = {407},
       number = {1},
        pages = {144-162},
          doi = {10.1111/j.1365-2966.2010.16938.x},
archivePrefix = {arXiv},
       eprint = {1004.4896},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.407..144T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%-----------------------------------------------------------------------%
%Discussion

@ARTICLE{schawinski+09,
       author = {{Schawinski}, Kevin and {Lintott}, Chris and {Thomas}, Daniel and {Sarzi}, Marc and {Andreescu}, Dan and {Bamford}, Steven P. and {Kaviraj}, Sugata and {Khochfar}, Sadegh and {Land}, Kate and {Murray}, Phil and {Nichol}, Robert C. and {Raddick}, M. Jordan and {Slosar}, An{\v{z}}e and {Szalay}, Alex and {VandenBerg}, Jan and {Yi}, Sukyoung K.},
        title = "{Galaxy Zoo: a sample of blue early-type galaxies at low redshift*}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: starburst, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = jun,
       volume = {396},
       number = {2},
        pages = {818-829},
          doi = {10.1111/j.1365-2966.2009.14793.x},
archivePrefix = {arXiv},
       eprint = {0903.3415},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.396..818S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lee+06,
       author = {{Lee}, Joon Hyeop and {Lee}, Myung Gyoon and {Hwang}, Ho Seong},
        title = "{The Nature of Blue Early-Type Galaxies in the GOODS Fields}",
      journal = {\apj},
     keywords = {Cosmology: Observations, Galaxies: Elliptical and Lenticular, cD, Galaxies: Evolution, Galaxies: Formation, Galaxies: Structure, Astrophysics},
         year = 2006,
        month = oct,
       volume = {650},
       number = {1},
        pages = {148-165},
          doi = {10.1086/507121},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606608},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...650..148L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kannappan+09,
       author = {{Kannappan}, Sheila J. and {Guie}, Jocelly M. and {Baker}, Andrew J.},
        title = "{E/S0 Galaxies on the Blue Color-Stellar Mass Sequence at z = 0: Fading Mergers or Future Spirals?}",
      journal = {\aj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2009,
        month = aug,
       volume = {138},
       number = {2},
        pages = {579-597},
          doi = {10.1088/0004-6256/138/2/579},
archivePrefix = {arXiv},
       eprint = {0903.3695},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009AJ....138..579K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vulcani+15,
       author = {{Vulcani}, Benedetta and {Poggianti}, Bianca M. and {Fritz}, Jacopo and {Fasano}, Giovanni and {Moretti}, Alessia and {Calvi}, Rosa and {Paccagnella}, Angela},
        title = "{From Blue Star-forming to Red Passive: Galaxies in Transition in Different Environments}",
      journal = {\apj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: fundamental parameters, galaxies: groups: general, galaxies: spiral, galaxies: star formation, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jan,
       volume = {798},
       number = {1},
          eid = {52},
        pages = {52},
          doi = {10.1088/0004-637X/798/1/52},
archivePrefix = {arXiv},
       eprint = {1410.6481},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798...52V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kaviraj+14,
       author = {{Kaviraj}, Sugata},
        title = "{The significant contribution of minor mergers to the cosmic star formation budget}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: interactions, galaxies: starburst, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = jan,
       volume = {437},
       number = {1},
        pages = {L41-L45},
          doi = {10.1093/mnrasl/slt136},
archivePrefix = {arXiv},
       eprint = {1310.0007},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.437L..41K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{liu+21,
       author = {{Liu}, Shuang and {Gu}, Yizhou and {Yuan}, Qirong and {Lu}, Shiying and {Bao}, Min and {Fang}, Guanwen and {Fan}, Lulu},
        title = "{Morphological Transformation and Star Formation Quenching of Massive Galaxies at 0.5 {\ensuremath{\leq}} z {\ensuremath{\leq}} 2.5 in 3D-HST/CANDELS}",
      journal = {\apj},
     keywords = {734, 2029, 615, 429, 907, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = dec,
       volume = {923},
       number = {1},
          eid = {46},
        pages = {46},
          doi = {10.3847/1538-4357/ac2817},
archivePrefix = {arXiv},
       eprint = {2110.12704},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923...46L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rin06,
   author = {{Rines}, K. and {Diaferio}, A.},
    title = "{CIRS: Cluster Infall Regions in the Sloan Digital Sky Survey. I. Infall Patterns and Mass Profiles}",
  journal = {\aj},
   eprint = {astro-ph/0602032},
 keywords = {Cosmology: Observations, Galaxies: Clusters: General, Galaxies: Kinematics and Dynamics},
     year = 2006,
    month = sep,
   volume = 132,
    pages = {1275-1297},
      doi = {10.1086/506017},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006AJ....132.1275R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rei02,
       author = {{Reiprich}, Thomas H. and {B{\"o}hringer}, Hans},
        title = "{The Mass Function of an X-Ray Flux-limited Sample of Galaxy Clusters}",
      journal = {\apj},
     keywords = {Cosmology: Cosmological Parameters, Cosmology: Observations, Galaxies: Clusters: General, Galaxies: Intergalactic Medium, Cosmology: Large-Scale Structure of Universe, X-Rays: Galaxies: Clusters, Astrophysics},
         year = 2002,
        month = mar,
       volume = {567},
       number = {2},
        pages = {716-740},
          doi = {10.1086/338753},
archivePrefix = {arXiv},
       eprint = {astro-ph/0111285},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...567..716R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pla11,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Balbi}, A. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartelmann}, M. and {Bartlett}, J.~G. and {Battaner}, E. and {Battye}, R. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bhatia}, R. and {Bock}, J.~J. and {Bonaldi}, A. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Brown}, M.~L. and {Bucher}, M. and {Burigana}, C. and {Cabella}, P. and {Cantalupo}, C.~M. and {Cardoso}, J. -F. and {Carvalho}, P. and {Catalano}, A. and {Cay{\'o}n}, L. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, L. -Y. and {Chiang}, C. and {Chon}, G. and {Christensen}, P.~R. and {Churazov}, E. and {Clements}, D.~L. and {Colafrancesco}, S. and {Colombi}, S. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Cuttaia}, F. and {da Silva}, A. and {Dahle}, H. and {Danese}, L. and {Davis}, R.~J. and {de Bernardis}, P. and {de Gasperis}, G. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {Dickinson}, C. and {Diego}, J.~M. and {Dolag}, K. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {D{\"o}rl}, U. and {Douspis}, M. and {Dupac}, X. and {Efstathiou}, G. and {Eisenhardt}, P. and {En{\ss}lin}, T.~A. and {Feroz}, F. and {Finelli}, F. and {Flores-Cacho}, I. and {Forni}, O. and {Fosalba}, P. and {Frailis}, M. and {Franceschi}, E. and {Fromenteau}, S. and {Galeotta}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Giard}, M. and {Giardino}, G. and {Giraud-H{\'e}raud}, Y. and {Gonz{\'a}lez-Nuevo}, J. and {Gonz{\'a}lez-Riestra}, R. and {G{\'o}rski}, K.~M. and {Grainge}, K.~J.~B. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Harrison}, D. and {Hein{\"a}m{\"a}ki}, P. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hovest}, W. and {Hoyland}, R.~J. and {Huffenberger}, K.~M. and {Hurier}, G. and {Hurley-Walker}, N. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knox}, L. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Laureijs}, R.~J. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Leach}, S. and {Leonardi}, R. and {Li}, C. and {Liddle}, A. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {MacTavish}, C.~J. and {Maffei}, B. and {Maino}, D. and {Mandolesi}, N. and {Mann}, R. and {Maris}, M. and {Marleau}, F. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {Matthai}, F. and {Mazzotta}, P. and {Mei}, S. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Melin}, J. -B. and {Mendes}, L. and {Mennella}, A. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Munshi}, D. and {Murphy}, A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Olamaie}, M. and {Osborne}, S. and {Pajot}, F. and {Pasian}, F. and {Patanchon}, G. and {Pearson}, T.~J. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Piffaretti}, R. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Poutanen}, T. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Renault}, C. and {Ricciardi}, S. and {Riller}, T. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Saar}, E. and {Sandri}, M. and {Santos}, D. and {Saunders}, R.~D.~E. and {Savini}, G. and {Schaefer}, B.~M. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, P. and {Smoot}, G.~F. and {Stanford}, A. and {Starck}, J. -L. and {Stivoli}, F. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sunyaev}, R. and {Sutton}, D. and {Sygnet}, J. -F. and {Taburet}, N. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Torre}, J. -P. and {Tristram}, M. and {Tuovinen}, J. and {Valenziano}, L. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Weller}, J. and {White}, S.~D.~M. and {White}, M. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck early results. VIII. The all-sky early Sunyaev-Zeldovich cluster sample}",
      journal = {\aap},
     keywords = {cosmology: observations, galaxies: clusters: general, catalogs, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = dec,
       volume = {536},
          eid = {A8},
        pages = {A8},
          doi = {10.1051/0004-6361/201116459},
archivePrefix = {arXiv},
       eprint = {1101.2024},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...536A...8P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kir21,
       author = {{Kirkpatrick}, C.~C. and {Clerc}, N. and {Finoguenov}, A. and {Damsted}, S. and {Ider Chitham}, J. and {Kukkola}, A.~E. and {Gueguen}, A. and {Furnell}, K. and {Rykoff}, E. and {Comparat}, J. and {Saro}, A. and {Capasso}, R. and {Padilla}, N. and {Erfanianfar}, G. and {Mamon}, G.~A. and {Collins}, C. and {Merloni}, A. and {Brownstein}, J.~R. and {Schneider}, D.~P.},
        title = "{SPIDERS: an overview of the largest catalogue of spectroscopically confirmed x-ray galaxy clusters}",
      journal = {\mnras},
     keywords = {catalogues, galaxies: clusters: general, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jun,
       volume = {503},
       number = {4},
        pages = {5763-5777},
          doi = {10.1093/mnras/stab127},
archivePrefix = {arXiv},
       eprint = {2101.04695},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.5763K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pin96,
       author = {{Pinkney}, Jason and {Roettiger}, Kurt and {Burns}, Jack O. and {Bird}, Christina M.},
        title = "{Evaluation of Statistical Tests for Substructure in Clusters of Galaxies}",
      journal = {\apjs},
     keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: DISTANCES AND REDSHIFTS, GALAXIES: INTERACTIONS, METHODS: NUMERICAL},
         year = 1996,
        month = may,
       volume = {104},
        pages = {1},
          doi = {10.1086/192290},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJS..104....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{conselice03,
       author = {{Conselice}, Christopher J.},
        title = "{The Relationship between Stellar Light Distributions of Galaxies and Their Formation Histories}",
      journal = {\apjs},
     keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: Structure, Astrophysics},
         year = 2003,
        month = jul,
       volume = {147},
       number = {1},
        pages = {1-28},
          doi = {10.1086/375001},
archivePrefix = {arXiv},
       eprint = {astro-ph/0303065},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJS..147....1C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sampaio+21,
       author = {{Sampaio}, V.~M. and {de Carvalho}, R.~R. and {Ferreras}, I. and {Lagan{\'a}}, T.~F. and {Ribeiro}, A.~L.~B. and {Rembold}, S.~B.},
        title = "{Investigating the projected phase space of Gaussian and non-Gaussian clusters}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxy: evolution, galaxy: formation, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {503},
       number = {2},
        pages = {3065-3080},
          doi = {10.1093/mnras/stab673},
archivePrefix = {arXiv},
       eprint = {2103.03030},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.3065S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{coccato+20,
       author = {{Coccato}, Lodovico and {Jaff{\'e}}, Yara L. and {Cortesi}, Arianna and {Merrifield}, Michael and {Johnston}, Evelyn and {Rodr{\'\i}guez del Pino}, Bruno and {Haeussler}, Boris and {Chies-Santos}, Ana L. and {Mendes de Oliveira}, Claudia L. and {Sheen}, Yun-Kyeong and {Men{\'e}ndez-Delmestre}, Kar{\'\i}n},
        title = "{Formation of S0s in extreme environments I: clues from kinematics and stellar populations}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = feb,
       volume = {492},
       number = {2},
        pages = {2955-2972},
          doi = {10.1093/mnras/stz3592},
archivePrefix = {arXiv},
       eprint = {1912.08845},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492.2955C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{coccato+22,
       author = {{Coccato}, Lodovico and {Fraser-McKelvie}, Amelia and {Jaff{\'e}}, Yara L. and {Johnston}, Evelyn J. and {Cortesi}, Arianna and {Pallero}, Diego},
        title = "{Formation of S0s in extreme environments III: the role of environment in the formation pathways}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: kinematics and dynamics, galaxies: stellar content, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = sep,
       volume = {515},
       number = {1},
        pages = {201-212},
          doi = {10.1093/mnras/stac1764},
archivePrefix = {arXiv},
       eprint = {2206.11915},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.515..201C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jaffe+16,
       author = {{Jaff{\'e}}, Yara L. and {Verheijen}, Marc A.~W. and {Haines}, Chris P. and {Yoon}, Hyein and {Cybulski}, Ryan and {Montero-Casta{\~n}o}, Mar{\'\i}a and {Smith}, Rory and {Chung}, Aeree and {Deshev}, Boris Z. and {Fern{\'a}ndez}, Ximena and {van Gorkom}, Jacqueline and {Poggianti}, Bianca M. and {Yun}, Min S. and {Finoguenov}, Alexis and {Smith}, Graham P. and {Okabe}, Nobuhiro},
        title = "{BUDHIES - III: the fate of H I and the quenching of galaxies in evolving environments}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: clusters: individual: Abell 963, galaxies: evolution, galaxies: interactions, galaxies: peculiar, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = sep,
       volume = {461},
       number = {2},
        pages = {1202-1221},
          doi = {10.1093/mnras/stw984},
archivePrefix = {arXiv},
       eprint = {1604.07832},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.461.1202J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hickson+97,
       author = {{Hickson}, Paul},
        title = "{Compact Groups of Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = 1997,
        month = jan,
       volume = {35},
        pages = {357-388},
          doi = {10.1146/annurev.astro.35.1.357},
archivePrefix = {arXiv},
       eprint = {astro-ph/9710289},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ARA&A..35..357H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{lotz+19,
       author = {{Lotz}, Marcel and {Remus}, Rhea-Silvia and {Dolag}, Klaus and {Biviano}, Andrea and {Burkert}, Andreas},
        title = "{Gone after one orbit: How cluster environments quench galaxies}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, galaxies: evolution, galaxies: clusters: general, galaxies: star formation, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = oct,
       volume = {488},
       number = {4},
        pages = {5370-5389},
          doi = {10.1093/mnras/stz2070},
archivePrefix = {arXiv},
       eprint = {1810.02382},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.488.5370L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{barchi+20,
       author = {{Barchi}, P.~H. and {de Carvalho}, R.~R. and {Rosa}, R.~R. and {Sautter}, R.~A. and {Soares-Santos}, M. and {Marques}, B.~A.~D. and {Clua}, E. and {Gon{\c{c}}alves}, T.~S. and {de S{\'a}-Freitas}, C. and {Moura}, T.~C.},
        title = "{Machine and Deep Learning applied to galaxy morphology - A comparative study}",
      journal = {Astronomy and Computing},
     keywords = {Galaxies: photometry, Methods: data analysis, Machine learning, Techniques: image processing, Galaxies: General, Catalogs, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
       volume = {30},
          eid = {100334},
        pages = {100334},
          doi = {10.1016/j.ascom.2019.100334},
archivePrefix = {arXiv},
       eprint = {1901.07047},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&C....3000334B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{sarazin-88,
       author = {{Sarazin}, Craig L.},
        title = "{X-Ray Emission from Clusters of Galaxies}",
         year = 2009,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009xecg.book.....S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zinger+18,
       author = {{Zinger}, Elad and {Dekel}, Avishai and {Kravtsov}, Andrey V. and {Nagai}, Daisuke},
        title = "{Quenching of satellite galaxies at the outskirts of galaxy clusters}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: clusters: intracluster medium, galaxies: evolution, galaxies: star formation},
         year = 2018,
        month = apr,
       volume = {475},
       number = {3},
        pages = {3654-3681},
          doi = {10.1093/mnras/stx3329},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.475.3654Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wang+18,
       author = {{Wang}, L. and {Norberg}, P. and {Brough}, S. and {Brown}, M.~J.~I. and {da Cunha}, E. and {Davies}, L.~J. and {Driver}, S.~P. and {Holwerda}, B.~W. and {Hopkins}, A.~M. and {Lara-Lopez}, M.~A. and {Liske}, J. and {Loveday}, J. and {Grootes}, M.~W. and {Popescu}, C.~C. and {Wright}, A.~H.},
        title = "{Galaxy and Mass Assembly (GAMA): The environmental dependence of the galaxy main sequence}",
      journal = {\aap},
     keywords = {galaxies: abundances, galaxies: star formation, galaxies: statistics, galaxies: evolution, galaxies: groups: general, galaxies: halos, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201832697},
archivePrefix = {arXiv},
       eprint = {1802.08456},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A...1W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{haines+13,
       author = {{Haines}, C.~P. and {Pereira}, M.~J. and {Smith}, G.~P. and {Egami}, E. and {Sanderson}, A.~J.~R. and {Babul}, A. and {Finoguenov}, A. and {Merluzzi}, P. and {Busarello}, G. and {Rawle}, T.~D. and {Okabe}, N.},
        title = "{LoCuSS: The Steady Decline and Slow Quenching of Star Formation in Cluster Galaxies over the Last Four Billion Years}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, galaxies: evolution, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = oct,
       volume = {775},
       number = {2},
          eid = {126},
        pages = {126},
          doi = {10.1088/0004-637X/775/2/126},
archivePrefix = {arXiv},
       eprint = {1307.1135},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...775..126H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lop17,
       author = {{Lopes}, P.~A.~A. and {Ribeiro}, A.~L.~B. and {Rembold}, S.~B.},
        title = "{NoSOCS in SDSS - VI. The environmental dependence of AGN in clusters and  field in the local Universe}",
      journal = {\mnras},
     keywords = {surveys, galaxies: clusters: general, galaxies: evolution, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = nov,
       volume = {472},
       number = {1},
        pages = {409-418},
          doi = {10.1093/mnras/stx2046},
archivePrefix = {arXiv},
       eprint = {1708.02242},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.472..409L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lop06,
       author = {{Lopes}, P.~A.~A. and {de Carvalho}, R.~R. and {Capelato}, H.~V. and {Gal}, R.~R. and {Djorgovski}, S.~G. and {Brunner}, R.~J. and {Odewahn}, S.~C. and {Mahabal}, A.~A.},
        title = "{X-Ray Galaxy Clusters in NoSOCS: Substructure and the Correlation of Optical and X-Ray Properties}",
      journal = {\apj},
     keywords = {Catalogs, Galaxies: Clusters: General, X-Rays: Galaxies, Astrophysics},
         year = 2006,
        month = sep,
       volume = {648},
       number = {1},
        pages = {209-229},
          doi = {10.1086/505630},
archivePrefix = {arXiv},
       eprint = {astro-ph/0605292},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...648..209L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lab10,
       author = {{La Barbera}, F. and {Lopes}, P.~A.~A. and {de Carvalho}, R.~R. and {de La Rosa}, I.~G. and {Berlind}, A.~A.},
        title = "{SPIDER - III. Environmental dependence of the Fundamental Plane of early-type galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: groups: general, galaxies: stellar content, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = nov,
       volume = {408},
       number = {3},
        pages = {1361-1386},
          doi = {10.1111/j.1365-2966.2010.17273.x},
archivePrefix = {arXiv},
       eprint = {1003.1119},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.408.1361L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kuc17,
       author = {{Kuchner}, U. and {Ziegler}, B. and {Verdugo}, M. and {Bamford}, S. and {H{\"a}u{\ss}ler}, B.},
        title = "{The effects of the cluster environment on the galaxy mass-size relation in MACS J1206.2-0847}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: clusters: individual: MACS J1206.2-0847, galaxies: clusters: general, galaxies: structure, galaxies: elliptical and lenticular, cD, galaxies: fundamental parameters, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = aug,
       volume = {604},
          eid = {A54},
        pages = {A54},
          doi = {10.1051/0004-6361/201630252},
archivePrefix = {arXiv},
       eprint = {1705.03839},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...604A..54K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mah18,
       author = {{Mahajan}, Smriti and {Drinkwater}, Michael J. and {Driver}, S. and {Hopkins}, A.~M. and {Graham}, Alister W. and {Brough}, S. and {Brown}, Michael J.~I. and {Holwerda}, B.~W. and {Owers}, Matt S. and {Pimbblet}, Kevin A.},
        title = "{Galaxy And Mass Assembly (GAMA): blue spheroids within 87 Mpc}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: star formation, galaxies: stellar content, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = mar,
       volume = {475},
       number = {1},
        pages = {788-799},
          doi = {10.1093/mnras/stx3202},
archivePrefix = {arXiv},
       eprint = {1712.03644},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.475..788M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balogh+99,
       author = {{Balogh}, Michael L. and {Morris}, Simon L. and {Yee}, H.~K.~C. and {Carlberg}, R.~G. and {Ellingson}, Erica},
        title = "{Differential Galaxy Evolution in Cluster and Field Galaxies at z\raisebox{-0.5ex}\textasciitilde0.3}",
      journal = {\apj},
     keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: EVOLUTION, GALAXIES: PHOTOMETRY, GALAXIES: STELLAR CONTENT, Galaxies: Clusters: General, Galaxies: Evolution, Galaxies: Photometry, Galaxies: Stellar Content, Astrophysics},
         year = 1999,
        month = dec,
       volume = {527},
       number = {1},
        pages = {54-79},
          doi = {10.1086/308056},
archivePrefix = {arXiv},
       eprint = {astro-ph/9906470},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...527...54B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{saglia+00,
       author = {{Saglia}, R.~P. and {Maraston}, C. and {Greggio}, L. and {Bender}, R. and {Ziegler}, B.},
        title = "{The evolution of the color gradients of early-type cluster galaxies}",
      journal = {\aap},
     keywords = {GALAXIES: ELLIPTICAL AND LENTICULAR, CD, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: ABUNDANCES, GALAXIES: FORMATION, Astrophysics},
         year = 2000,
        month = aug,
       volume = {360},
        pages = {911-934},
archivePrefix = {arXiv},
       eprint = {astro-ph/0007038},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...360..911S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kobayashi-04,
       author = {{Kobayashi}, Chiaki},
        title = "{GRAPE-SPH chemodynamical simulation of elliptical galaxies - I. Evolution of metallicity gradients}",
      journal = {\mnras},
     keywords = {methods: N-body simulations, galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, Astrophysics},
         year = 2004,
        month = jan,
       volume = {347},
       number = {3},
        pages = {740-758},
          doi = {10.1111/j.1365-2966.2004.07258.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0310160},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.347..740K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tamura+00a,
       author = {{Tamura}, Naoyuki and {Kobayashi}, Chiaki and {Arimoto}, Nobuo and {Kodama}, Tadayuki and {Ohta}, Kouji},
        title = "{Origin of Color Gradients in Elliptical Galaxies}",
      journal = {\aj},
     keywords = {GALAXIES: ELLIPTICAL AND LENTICULAR, CD, GALAXIES: EVOLUTION, GALAXIES: FORMATION, Astrophysics},
         year = 2000,
        month = may,
       volume = {119},
       number = {5},
        pages = {2134-2145},
          doi = {10.1086/301333},
archivePrefix = {arXiv},
       eprint = {astro-ph/0001174},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000AJ....119.2134T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tamura+00b,
       author = {{Tamura}, Naoyuki and {Ohta}, Kouji},
        title = "{Color Gradients in Early-Type Galaxies in Clusters at Redshift 0.37-0.56}",
      journal = {\aj},
     keywords = {Galaxies: Elliptical and Lenticular, cD, Galaxies: Evolution, Galaxies: Formation, Astrophysics},
         year = 2000,
        month = aug,
       volume = {120},
       number = {2},
        pages = {533-539},
          doi = {10.1086/301460},
archivePrefix = {arXiv},
       eprint = {astro-ph/0004221},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000AJ....120..533T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meert+15,
       author = {{Meert}, Alan and {Vikram}, Vinu and {Bernardi}, Mariangela},
        title = "{A catalogue of 2D photometric decompositions in the SDSS-DR7 spectroscopic main galaxy sample: preferred models and systematics}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {446},
       number = {4},
        pages = {3943-3974},
          doi = {10.1093/mnras/stu2333},
archivePrefix = {arXiv},
       eprint = {1406.4179},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446.3943M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meert+16,
       author = {{Meert}, Alan and {Vikram}, Vinu and {Bernardi}, Mariangela},
        title = "{A catalogue of two-dimensional photometric decompositions in the SDSS-DR7 spectroscopic main galaxy sample: extension to g and I bands}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = jan,
       volume = {455},
       number = {3},
        pages = {2440-2452},
          doi = {10.1093/mnras/stv2475},
archivePrefix = {arXiv},
       eprint = {1510.07631},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.455.2440M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rib13,
       author = {{Ribeiro}, A.~L.~B. and {Lopes}, P.~A.~A. and {Rembold}, S.~B.},
        title = "{NoSOCS in SDSS. III. The interplay between galaxy evolution and the dynamical state of galaxy clusters}",
      journal = {\aap},
     keywords = {galaxies: clusters: general, galaxies: evolution, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {556},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201220801},
archivePrefix = {arXiv},
       eprint = {1306.6935},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...556A..74R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gir98,
       author = {{Girardi}, Marisa and {Giuricin}, Giuliano and {Mardirossian}, Fabio and {Mezzetti}, Marino and {Boschin}, Walter},
        title = "{Optical Mass Estimates of Galaxy Clusters}",
      journal = {\apj},
     keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: FUNDAMENTAL PARAMETERS, X-RAYS: GALAXIES, Galaxies: Clusters: General, Galaxies: Fundamental Parameters, X-Rays: Galaxies, Astrophysics},
         year = 1998,
        month = sep,
       volume = {505},
       number = {1},
        pages = {74-95},
          doi = {10.1086/306157},
archivePrefix = {arXiv},
       eprint = {astro-ph/9804187},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...505...74G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fer20,
       author = {{Ferragamo}, A. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Betancort-Rijo}, J. and {Munari}, E. and {Sartoris}, B. and {Barrena}, R.},
        title = "{Biases in galaxy cluster velocity dispersion and mass estimates in the small N$_{gal}$ regime}",
      journal = {\aap},
     keywords = {large-scale structure of Universe, galaxies: clusters: general, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A41},
        pages = {A41},
          doi = {10.1051/0004-6361/201834837},
archivePrefix = {arXiv},
       eprint = {2006.05949},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A..41F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{car97,
       author = {{Carlberg}, R.~G. and {Yee}, H.~K.~C. and {Ellingson}, E.},
        title = "{The Average Mass and Light Profiles of Galaxy Clusters}",
      journal = {\apj},
     keywords = {Galaxies: Clusters: General, Galaxies: Kinematics and Dynamics, Galaxies: Photometry, Astrophysics},
         year = 1997,
        month = mar,
       volume = {478},
       number = {2},
        pages = {462-475},
          doi = {10.1086/303805},
archivePrefix = {arXiv},
       eprint = {astro-ph/9512087},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...478..462C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mun13,
       author = {{Munari}, E. and {Biviano}, A. and {Borgani}, S. and {Murante}, G. and {Fabjan}, D.},
        title = "{The relation between velocity dispersion and mass in simulated clusters of galaxies: dependence on the tracer and the baryonic physics}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: clusters: general, galaxies: evolution, galaxies: groups: general, galaxies: kinematics and dynamics, cosmology: theory, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2013,
        month = apr,
       volume = {430},
       number = {4},
        pages = {2638-2649},
          doi = {10.1093/mnras/stt049},
archivePrefix = {arXiv},
       eprint = {1301.1682},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.430.2638M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pop07,
       author = {{Popesso}, P. and {Biviano}, A. and {B{\"o}hringer}, H. and {Romaniello}, M.},
        title = "{RASS-SDSS galaxy cluster survey. VII. On the cluster mass-to-light ratio and the halo occupation distribution}",
      journal = {\aap},
     keywords = {galaxies: clusters: general, galaxies: luminosity function, mass function, Astrophysics},
         year = 2007,
        month = mar,
       volume = {464},
       number = {2},
        pages = {451-464},
          doi = {10.1051/0004-6361:20054708},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606260},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...464..451P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kau03b,
       author = {{Kauffmann}, Guinevere and {Heckman}, Timothy M. and {White}, Simon D.~M. and {Charlot}, St{\'e}phane and {Tremonti}, Christy and {Peng}, Eric W. and {Seibert}, Mark and {Brinkmann}, Jon and {Nichol}, Robert C. and {SubbaRao}, Mark and {York}, Don},
        title = "{The dependence of star formation history and internal structure on stellar mass for {}10$^{5}$ low-redshift galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = may,
       volume = {341},
       number = {1},
        pages = {54-69},
          doi = {10.1046/j.1365-8711.2003.06292.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205070},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.341...54K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{peletier+90,
       author = {{Peletier}, Reynier F. and {Davies}, Roger L. and {Illingworth}, Garth D. and {Davis}, Lindsey E. and {Cawson}, Michael},
        title = "{CCD Surface Photometry of Galaxies with Dynamical Data. II. UBR Photometry of 39 Elliptical Galaxies}",
      journal = {\aj},
     keywords = {Astronomical Photometry, Brightness Distribution, Elliptical Galaxies, Galactic Evolution, Galactic Structure, Ultraviolet Photometry, Charge Coupled Devices, Color-Color Diagram, Seeing (Astronomy), Astronomy, GALAXIES: PHOTOMETRY, GALAXIES: SURFACE},
         year = 1990,
        month = oct,
       volume = {100},
        pages = {1091},
          doi = {10.1086/115582},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990AJ....100.1091P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{palmese+17,
       author = {{Palmese}, A. and {Hartley}, W. and {Tarsitano}, F. and {Conselice}, C. and {Lahav}, O. and {Allam}, S. and {Annis}, J. and {Lin}, H. and {Soares-Santos}, M. and {Tucker}, D. and {Brout}, D. and {Banerji}, M. and {Bechtol}, K. and {Diehl}, H.~T. and {Fruchter}, A. and {Garc{\'\i}a-Bellido}, J. and {Herner}, K. and {Levan}, A.~J. and {Li}, T.~S. and {Lidman}, C. and {Misra}, K. and {Sako}, M. and {Scolnic}, D. and {Smith}, M. and {Abbott}, T.~M.~C. and {Abdalla}, F.~B. and {Benoit-L{\'e}vy}, A. and {Bertin}, E. and {Brooks}, D. and {Buckley-Geer}, E. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Cunha}, C.~E. and {D'Andrea}, C.~B. and {da Costa}, L.~N. and {Davis}, C. and {DePoy}, D.~L. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Drlica-Wagner}, A. and {Eifler}, T.~F. and {Evrard}, A.~E. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruen}, D. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Honscheid}, K. and {Jain}, B. and {James}, D.~J. and {Jeltema}, T. and {Johnson}, M.~W.~G. and {Johnson}, M.~D. and {Krause}, E. and {Kron}, R. and {Kuehn}, K. and {Kuhlmann}, S. and {Kuropatkin}, N. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {McMahon}, R.~G. and {Menanteau}, F. and {Miller}, C.~J. and {Miquel}, R. and {Neilsen}, E. and {Ogando}, R.~L.~C. and {Plazas}, A.~A. and {Reil}, K. and {Romer}, A.~K. and {Sanchez}, E. and {Schindler}, R. and {Smith}, R.~C. and {Sobreira}, F. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {Thomas}, R.~C. and {Walker}, A.~R. and {Weller}, J. and {Zhang}, Y. and {Zuntz}, J.},
        title = "{Evidence for Dynamically Driven Formation of the GW170817 Neutron Star Binary in NGC 4993}",
      journal = {\apjl},
     keywords = {galaxies: individual: NGC 4993, galaxies: evolution, galaxies: structure, gravitational waves, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = nov,
       volume = {849},
       number = {2},
          eid = {L34},
        pages = {L34},
          doi = {10.3847/2041-8213/aa9660},
archivePrefix = {arXiv},
       eprint = {1710.06748},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...849L..34P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rib11,
       author = {{Ribeiro}, A.~L.~B. and {Lopes}, P.~A.~A. and {Trevisan}, M.},
        title = "{Non-Gaussian velocity distributions - the effect on virial mass estimates of galaxy groups}",
      journal = {\mnras},
     keywords = {galaxies: groups: general, galaxies: statistics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = may,
       volume = {413},
       number = {1},
        pages = {L81-L85},
          doi = {10.1111/j.1745-3933.2011.01038.x},
archivePrefix = {arXiv},
       eprint = {1103.0426},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.413L..81R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


